EnGN: A High-Throughput and Energy-Efficient Accelerator for Large Graph Neural Networks

Graph neural networks (GNNs) emerge as a powerful approach to process non-euclidean data structures and have been proved powerful in various application domains such as social networks and e-commerce. While such graph data maintained in real-world systems can be extremely large and sparse, thus employing GNNs to deal with them requires substantial computational and memory overhead, which induces considerable energy and resource cost on CPUs and GPUs. In this work, we present a specialized accelerator architecture, EnGN, to enable high-throughput and energy-efficient processing of large-scale GNNs. The proposed EnGN is designed to accelerate the three key stages of GNN propagation, which is abstracted as common computing patterns shared by typical GNNs. To support the key stages simultaneously, we propose the ring-edge-reduce(RER) dataflow that tames the poor locality of sparsely-and-randomly connected vertices, and the RER PE-array to practice RER dataflow. In addition, we utilize a graph tiling strategy to fit large graphs into EnGN and make good use of the hierarchical on-chip buffers through adaptive computation reordering and tile scheduling. Overall, EnGN achieves performance speedup by 1802.9X, 19.75X, and 2.97X and energy efficiency by 1326.35X, 304.43X, and 6.2X on average compared to CPU, GPU, and a state-of-the-art GCN accelerator HyGCN, respectively.

==> Section/Engn_architecture_backup.tex <==
\section{EnGN Architecture}
\subsection{EnGN hardware architecture}
%It roughly consists of three major types of components including computing components, on-chip memory components and control components.
%Computing components are responsible for the different computing tasks in EnGN model and mainly include a neural graph processing units (NGGPU), 
%a vector processing unit, a non-linear activation processing unit (XPE). NGGPU is the key computing unit and is used for the majority 
%of the computing in $feature\_extraction()$ and $aggregation()$. With 2D array interconnection, matrix computing 
%in $feature\_extraction()$ can be mapped efficiently on NGGPU. With additional ring interconnection, reduced accumulation in each row of 
%NGGPU can be performed on NGGPU as well. While there may also \cheng{xxx} processing required in some of 
%the $feature\_extraction()$ as presented in \cheng{ Table xxx}, we have them 
%implemented on the vector processing unit without stalling the computing on NGGPU. Finally, XPE is mainly used for the various non-linear 
%activation functions in $update()$. On-chip memory components mainly include property buffer, weight buffer, edge buffer 
%and result buffer, which are used to bridge the bandwidth gap between DRAM and the computing requirements by taking advantage of 
%the data locality. Property buffer is used to store the property of source vertex and destination vertex, 
%the Weight buffer is used to keep the learned GNN parameters associated with the feature extraction and update function, 
%the Edge buffer is for storing the input graph or subgraph partitions loaded from off-chip memory, and finally the 
%Result buffer is used to place the property of vertex generated from the aggregate and update function. 
%In addition, there is also small yet fast degree-aware cache. It can be used to store the data items that are frequently 
%accessed in these big on-chip buffers such as property buffer and can reduce accesses on the big on-chip buffers. 
%On top of the data buffers, instruction buffer that defines the coarse-grained processing sequence of EnGN is also utilized. 
%The control components include graph format converter, instruction decoder, DMA, and prefetch. Graph format converter is used as online 
%graph format conversion to ensure EnGN to support the typical graph representations of CSR and CSC in addition to COO. Instruction decoder is 
%used to decode the instructions and generate synchronized control signals for the overall EnGN execution. DMA is mainly used for efficient 
%block data movements between on-chip buffer and DRAM. Prefetch is used to preload input data to overlap the data loading the EnGN computing.
On top of the unified EnGN processing model, we develop a customized EnGN accelerator as shown in~\autoref{fig:EnGN hardware architecture}. 
It integrates a neural graph processing unit (NGPU) to perform Feature extraction, Aggregate, and Update operation in a unified architecture. It has an array of homogeneous processing elements (PE) and the array size is $32\times32$. Each PE unit contains a local register file to store the temporary results and act as intermediate for inter-PE communication. Each PE in the same column of the Ring-Edge-Reduce (RER) array is connected to its neighbors in a ring network to perform aggregate operation and each PE in the same row of the RER array can process a vertex property, which means the NGPU can process 32 vertices simultaneously. However, such processing parallelism requires substantial memory bandwidth. Thereby, to avoid performance degradation, EnGN optimizes the memory access pattern for vertex data and edge data moving. For source vertex data access in the large graph, we adopt the graph tiling technique and make the source vertex fetching only induces accesses to the continuous memory addresses. For random destination vertex accesses in the aggregate and update stage, EnGN leverages the hashed edge data layout and multi-level cache method to avoid write conflicts and improve data hit rate in the compact on-chip buffer. During processing, to generate the PE control signal, the PE controller of NGPU reads the edge list of the graph from the edge banks and parses it into bit-stream that controls the PE-array to perform inter-row aggregate operation (\ding{172} in~\autoref{fig:EnGN hardware architecture}). In addition, as shown in~\autoref{fig:EnGN hardware architecture}, each PE in the NGPU is attached by an XPE to perform activation functions, bias operation, and rounding operation in the update stage. There also exists on the chip a vector processing unit (VPU), which is used to deal with different feature extraction, aggregate and update functions of GNNs illustrated in~\autoref{table:GNN algorithms on GNN framework}. 
\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_Accelerator_Architecture.eps}
\caption{EnGN hardware architecture.}
\label{fig:EnGN hardware architecture}
\vspace{-5pt}
\end{figure}

\subsubsection{The RER PE array}
The feature extraction stage maps the high dimensions property of vertices to the low dimensions by using the learned weight matrix, and this stage is simply matrix multiplication operation. Thus, EnGN modifies the classical systolic array architecture to perform the feature extraction stage in NGPU. As shown in~\autoref{fig:Architecture details}, in order to handle arbitrary-dimension property of GNN algorithms, we propose the graph property aware (GPA) dataflow to decouple the input property of the vertex and the hardware computing structure. In this manner, each PE in the same column of PE-array is responsible for a single dimension of vertex property and each PE in the same row handles a single vertex. The properties of a vertex are arranged in columns and aligned in the property bank. The dimensions of input vertex property become independent to the hardware architecture and can be continuously injected to the PE-array regardless of the array size and the property dimension. However, as shown in~\autoref{fig:Architecture details}, each column is responsible for generating one dimension of output property while the dimension of output property is determined by the GNN models. Thereby, when the column size of the weight matrix is larger than that of the PE-array, we choose to split the weight matrix into partitions that match the column size of PE-array. For example,~\autoref{fig:Architecture details} depicts the weight matrix with 6 columns and 5 rows while the column size of PE-array is 3, where the row size of weight matrix depends on 5-d property of input vertex and the column size of weight matrix is determined by the target GNN model. In this case, the weight matrix is split by column into two parts to match the column size of PE-array. After that, the two pieces of weight sub-matrix are placed in the weight banks in the order of rows. In this manner, the processing unit can handle vertex with arbitrary dimension property.
\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_EnGN_hardware_details.eps}
\caption{Architecture details.}
\label{fig:Architecture details}
\vspace{-6pt}
\end{figure}
\subsubsection{The Ring Edge Reduce topology for PE communication} 
The aggregate procedure needs to collect the information according to the edge information. Thereby, as shown in~\autoref{fig:Architecture details}, each row of the PE-array in NGPU possesses a dedicated edge bank and each PE in the same row receives the same control signal parsed from edge list in the graph to gather the corresponding vertex property. Meanwhile, because each PE needs to broadcast its own vertex features generated by the feature extraction stage to all other PEs in the same column, aggregating the received information simultaneously can result in a large amount of hardware resource consumption. Thereby, inspired by the ring-all-reduce concept~\cite{ringreduce}, we propose the ring-edge-reduce (RER) aggregate dataflow to conduct aggregate stage inside the PE array instead of moving the data out to the buffer. As shown in~\autoref{fig:Architecture details}, because each column of PE performs the same operations without any communication in between, each PE in the same column of array is connected to its neighbors through an on-chip network of ring topology. Each PE in the same column only communicates with its two nearest neighbors (north, south). In our design, the PE sends its information to the northern neighbors and receives the information sent from the southern neighbors for property aggregating. In this manner, a PE can select the relevant vertices to aggregate based on the control signal parsed from the edges during the information flow between the PEs.
\subsubsection{The On-chip Memory Hierarchy}

\

\noindent \textbf{PE register file} The register files (RF) equipped in the PEs are divided into four groups including source vertex groups(SRC RF), destination vertex groups (DST RF), and two shadow groups (Shadow RF), which is depicted in~\autoref{fig:Memory hierarchy}. The SRC RF stores the source vertex values generated in the feature extraction stage. The DST RF stores the destination vertex feature updated during the aggregate and update stages. In addition, there are two programmer-invisible Shadow RFs holding the SRC and DST vertex values previously generated by the PEs of the same column, which work together with the DST and SRC RFs in a ping-pong way. 
\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/5_level_cache.eps}
\caption{Memory hierarchy.}
\label{fig:Memory hierarchy}
\vspace{-7pt}
\end{figure}

\noindent \textbf{Multiple-level caches} The real world graph has up to millions of vertices. Although the graph tiling technique adopted by EnGN helps fit the sub-graphs into the on-chip buffer, the set of vertices in the sub-graphs will still outsize the register files of the PE array. Meanwhile, the result banks are used to store the temporary aggregate results. PE frequently accesses the long-latency result bank will result in performance degradation. Thus, to improve the throughput of EnGN, as shown in~\autoref{fig:Memory hierarchy}, we insert a degree aware vertex cache (DAVC) between the result banks and the register file of each PE to improve the performance of the EnGN. The register file, DAVC, and the result banks are regarded as the first, second, and last level memories on chip, respectively. DAVC is a direct-mapped cache with the write-back policy and cache hit time of one cycles. DAVC uses the destination vertex id of edges as the line tag to determine whether the access to the vertex data hit or not in the DAVC. If hit, the vertex data will be directly read to DST RF in the PE unit. Otherwise, EnGN will access the last-level result banks. DAVC adopts the least recently used (LRU) replacement policy~\cite{LRU}. In this manner, the DAVC can alleviate the overhead incurred by the result bank accesses. EnGN also allocates a small space in the DAVC to cache some of the vertices with high-degree to reduce the on-chip memory traffics and the memory bandwidth required by the vertex data refetch because of the power-law distribution in the real-world graph. Since EnGN adopts graph tiling methods with a deterministic strategy, the vertex access can be predicted in advance. Thereby, EnGN provides a prefetcher unit to prefetch the vertices from off-chip memory to replace the property of vertex resides in the result banks as long as the all edges associated with the hold vertex are processed.

%For example, as shown in~\autoref{fig:Memory hierarchy}, suppose the compute array is sized at $1\times3$, EnGN needs to process the $(1,12)$, $(2,18)$, $(0,21)$, and $(1,24)$ edges. Because the number of the destination vertex of these edges can be divided by three, these edges are assigned to the first row $PE(0,0)$. The first edge $(1,12)$ can be directly processed in $PE(0,0)$ because the vertex 12 ($V_{12}$) is hit in the register file. The second edge $(2,18)$ in $PE(0,0)$ entails the access to the result bank because the vertex 18 ($V_{18}$) is not hit in the register file of $PE(0,0)$ and DAVC. In this case, DAVC will read a data chunk that contains multiple vertices from the result bank for better spatial locality. After that, when edge $(0,21)$ is accessed, PE can directly fetch data from DAVC without accessing the result bank with two cycle latency. 

%Considering the real-world graphs are highly skewed and generally follow the power-law distribution and the paper~\cite{AliGraph} also has proven that caching a small number of vertices with high-degree can achieve a significant cost decrease of graph traversals. Thereby, EnGN allocates a small space in the DAVC to cache some of the vertices with high-degree to reduce the off-chip memory traffics and the memory bandwidth required by the vertex data refetch. Meanwhile, Since EnGN splits the large-graph into 2-D partitions with a deterministic strategy, the vertex access can be predicted in advance. Thereby, EnGN provides a prefetcher unit to prefetch the vertices from off-chip memory to replace the property of vertex resides in the result banks as long as the all edges associated with the hold vertex are processed.
%These vertices with high-degree are prefetched from the off-chip memory to DAVC before a graph iteration begins. Until the end of a graph iteration, the data of these vertices with high-degree are written back to off-chip memory.

\noindent\textbf{Edge Bank} EnGN adopts graph tiling technique to divide the large graph into intervals and shards~\autoref{sec:graphtiling}. The edges of each shards are divided into different bank using modulo function according to the destination vertex id and the PE array size (\textbf{Edge Hash}), which is shown in~\autoref{fig:Architecture details}. For example, edges $(v_{5}, v_{0})$, $(v_{5}, v_{1})$, $(v_{5}, v_{2})$ will be placed into Row-1, Row-2, and Row-3 of the PE array, respectively. In this manner, each bank is only responsible for some dedicated edges and vertices update operations, heavy write conflicts due to simultaneous updates to the same vertex in different PEs can also be avoided. Meanwhile, we also rearrange the order of the edges within a shards based on the flow direction of the data in the ring topology to avoid redundant data traffics in the ring and improve the processing throughput of the edges.
%since EnGN adopts a ring-edge-reduce strategy to perform the aggregate stage, the processing order of edges within a shard must be orchestrated to avoid redundant data traffics in the ring and improve the processing throughput of the edges. For this reason, we rearrange the order of the edges within a shard according to the flow direction of the data in the ring topology. Edges are firstly sorted by the destination vertex and then sorted by the source vertex. After that, all edges with the same destination vertex in a PE unit are rearrange based on the order of the source vertex arriving at the PE. In this manner, when data flows in the ring, EnGN can guarantee that all edges can be handled in time.

%\begin{figure*}[!t]
%\centering
%%\setlength{\belowcaptionskip}{-10pt}
%\includegraphics[width=2.1\columnwidth]{Image/4_Neural_Graph_processing_model_in_EnGN.eps}
%\caption{Neural graph processing model in EnGN.}
%\label{fig:Neural graph processing model in EnGN}
%\end{figure*}	

\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_Dataflow_on_EnGn.eps}
\caption{EnGN Dataflow.}
\label{fig:EnGN Dataflow}
\vspace{-5pt}
\end{figure}

\subsection{EnGN dataflow}
We present in~\autoref{fig:EnGN Dataflow} an example to illustrate the execution flow of a GNN layer on the proposed EnGN hardware architecture based on GCN model~\cite{GCN}. Similar to the EnGN processing model, the execution stage of one GNN layer on the accelerator is also divided into three stages: feature extraction, aggregate, and update stage. The feature extraction and aggregate stage are executed in a pipelined manner while the update stage can only be triggered when the aggregate stage is completed. Without losing generality, as shown in~\autoref{fig:Architecture details} we consider a small design that consists of $4\times3$ PEs and the input graph is the same as the~\autoref{fig:EnGN processing model}. For brevity, we only describe the flow at the $PE(0,0)$ and $PE(1,0)$.

\textbf{Feature extraction:} At Cycle 0, $PE(0,0)$ receives the first dimension of the input vertex $V_0$ property $I(0,0)$ at the layer $l-1$, and the weight data $W(0,0)$ to generate the temporary property result $P(0,0)$. The result are stored in the local register file. 

At cycle 1, $PE(0,0)$ receives the second dimensions of input vertex $V_0$ property $I(0,1)$ and the weight data $W(1,0)$. Both of them are used to update the temporary property result $P(0,0)$.

On the follow-up cycles, the operations on $PE(0,0)$ are similar to cycle 1. The following new input properties $I(0,2)$, $I(0,3)$, $I(0,4)$ and the associated weight data $W(2,0)$, $W(3,0)$, $W(4,0)$ continuously feed into $PE(0,0)$ until the dimensions of vertices have been covered.

At cycle 4, the result $P(0,0)$ is generated and stored into the register file, waiting to be used by the aggregate stage. 

\textbf{Aggregate:} At cycle 5, Since the edge buffer contains vertex 0, $PE(0,0)$ uses $P(0,0)$ to generate the aggregate result $A(0,0)$. At the same time, $PE(0,0)$ sends $P(0,0)$ to $PE(3,0)$ and prepares for receiving the $P(1,0)$ sent from $PE(1,0)$.

At cycle 6, although $PE(0,0)$ receives $P(1,0)$ from $PE(1,0)$, $P(1,0)$ will not be utilized to update $A(0,0)$ because vertex 1 does not exist in the according edge list provided by the edge buffer, which means vertex 1 is not connected to vertex 0. Meanwhile, $PE(0,0)$ send $P(1,0)$ to $PE(3,0)$ and prepares for receiving $P(2,0)$ sent from $PE(1,0)$.

At cycle 7, $PE(0,0)$ receives $P(2,0)$ from $PE(1,0)$ and leverages it to update the aggregate result $A(0,0)$ because vertex 2 is in the according edge list provided by the edge buffer. Meanwhile, $P(2,0)$ is sent to $PE(3,0)$.

At cycle 8, $PE(0,0)$ receives $P(3,0)$ from $PE(1,0)$ and leverages it to update the aggregate result $A(0,0)$. In this case, all vertices have been traversed by each PE. Thus, $A(0,0)$ summarizes all the relevant edge information and will be stored in the register file to wait for the update stage.

\textbf{Update:} At cycle 9, since all edges associated with vertex 0 has been traversed, the aggregate result $A(0,0)$  will not be changed. Thereby, the update stage is triggered, and the aggregate result $A(0,0)$ is processed by the user-defined apply function, i.e. activation function $ReLu(\cdot)$ in GCNs, to generate the result $O(0,0)$ as the input to the next layer $l$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{EnGN Architecture}
\subsection{EnGN hardware architecture}
%It roughly consists of three major types of components including computing components, on-chip memory components and control components.
%Computing components are responsible for the different computing tasks in EnGN model and mainly include a neural graph processing units (NGGPU), 
%a vector processing unit, a non-linear activation processing unit (XPE). NGGPU is the key computing unit and is used for the majority 
%of the computing in $feature\_extraction()$ and $aggregation()$. With 2D array interconnection, matrix computing 
%in $feature\_extraction()$ can be mapped efficiently on NGGPU. With additional ring interconnection, reduced accumulation in each row of 
%NGGPU can be performed on NGGPU as well. While there may also \cheng{xxx} processing required in some of 
%the $feature\_extraction()$ as presented in \cheng{ Table xxx}, we have them 
%implemented on the vector processing unit without stalling the computing on NGGPU. Finally, XPE is mainly used for the various non-linear 
%activation functions in $update()$. On-chip memory components mainly include property buffer, weight buffer, edge buffer 
%and result buffer, which are used to bridge the bandwidth gap between DRAM and the computing requirements by taking advantage of 
%the data locality. Property buffer is used to store the property of source vertex and destination vertex, 
%the Weight buffer is used to keep the learned GNN parameters associated with the feature extraction and update function, 
%the Edge buffer is for storing the input graph or subgraph partitions loaded from off-chip memory, and finally the 
%Result buffer is used to place the property of vertex generated from the aggregate and update function. 
%In addition, there is also small yet fast degree-aware cache. It can be used to store the data items that are frequently 
%accessed in these big on-chip buffers such as property buffer and can reduce accesses on the big on-chip buffers. 
%On top of the data buffers, instruction buffer that defines the coarse-grained processing sequence of EnGN is also utilized. 
%The control components include graph format converter, instruction decoder, DMA, and prefetch. Graph format converter is used as online 
%graph format conversion to ensure EnGN to support the typical graph representations of CSR and CSC in addition to COO. Instruction decoder is 
%used to decode the instructions and generate synchronized control signals for the overall EnGN execution. DMA is mainly used for efficient 
%block data movements between on-chip buffer and DRAM. Prefetch is used to preload input data to overlap the data loading the EnGN computing.
On top of the unified EnGN processing model, we develop a customized EnGN accelerator as shown in~\autoref{fig:EnGN hardware architecture}. 
It integrates a neural graph processing unit (NGPU) to perform Feature extraction, Aggregate, and Update operation in a unified architecture. It has an array of homogeneous processing elements (PE) and the array size is $128 \times 16$. Each PE unit contains a local register file to store the temporary results and act as intermediate for inter-PE communication. Each PE in the same column of the Ring-Edge-Reduce (RER) array is connected to its neighbors in a ring network to perform aggregate operation and each PE in the same row of the RER array can process a vertex property, which means the NGPU can process 128 vertices simultaneously. However, such processing parallelism requires substantial memory bandwidth. Thereby, to avoid performance degradation, EnGN optimizes the memory access patterns for vertex data and edge data moving. For source vertex data access in the large graph, we adopt the graph tiling technique and ensure that the source vertex fetching only induces accesses to the continuous memory addresses. For random destination vertex accesses in the aggregate and update stage, EnGN leverages the hashed edge data layout and multi-level cache method to avoid write conflicts and improve data hit rate in the compact on-chip buffer. During processing, to generate the PE control signals, the PE controller of NGPU reads the edge list of the graph from the edge banks and parses it into bit-stream that controls the PE-array to perform inter-row aggregate operation (\ding{172} in~\autoref{fig:EnGN hardware architecture}). In addition, as shown in~\autoref{fig:EnGN hardware architecture}, each PE in the NGPU is attached by an XPE to perform activation functions, bias operation, and rounding operation in the update stage. A vector processing unit (VPU) is used to deal with different feature extraction, aggregate and update functions of GNNs illustrated in~\autoref{table:GNN algorithms on GNN framework}. There are also two auxiliary modules i.e. Prefetcher and Format converter that can be used to assist the memory accesses and improve the input graph format compatibility respectively.

\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_Accelerator_Architecture.eps}
\caption{EnGN hardware architecture.}
\label{fig:EnGN hardware architecture}
\vspace{-5pt}
\end{figure}

\subsection{GNN dataflow exploration}
Although EnGN accelerator built based on the unified EnGN processing framework allows developers to map various GNN algorithms on accelerator easily, the dataflow in accelerator still needs to be fully explored to achieve high-throughput and low-latency GNN processing. As summarized in ~\autoref{table:GNN algorithms on GNN framework}, matrix-matrix multiplication (MMM) used in both feature extraction and update phases and graph aggregate in the aggregate phase are the most time-consuming operations, so we mainly optimize the dataflows for the two operations to ensure efficient GNN processing on the accelerator. %The high-level feature extraction operation of the neural network and iterative graph aggregate are two important operations of GNN algorithms. The key operation of the feature extraction is essentially matrix-matrix multiplication.  

For MMM, the dataflow targeting at a regular 2D array has been intensively studied and there are three main options including \textit{Weight Stationary}, \textit{Output Stationary} and \textit{No Local Reuse}. The different dataflows mainly differ on the computing array utilization and the buffer bandwidth requirements. The best dataflow depends on both the 2D computing array size and the matrix size. Weight stationary maximizes the weight data reuse, but it can lead to under-utilization of the computing array when the feature dimensions are not aligned with the computing array. No Local Reuse poses high internal bandwidth requirement and causes massive internal data movement and energy consumption. In contrast, output stationary that explores both the inter-row and inter-column data reuse has much smaller buffer bandwidth requirements, but the computing array utilization is relatively lower in some cases. Unlike an independent MMM with determined matrix size, the MMM in GNNs may have distinct matrix size in different iterations because it is related with the the feature dimensions. The dataflow for MMM in GNNs needs to take the variation into consideration. For aggregate that conducts on a large sparse graph, the dataflow needs to aware both the data locality and the computing imbalance caused by the inherent graph irregularity. For higher performance of the overall GNNs, we propose a graph property aware dataflow for the MMM and ring edge reduce dataflow for the aggregate. The details will be illustrated in the next subsections. 
%There is no data hazard between the feature extraction and aggregate stage, so the two dataflows can be pipelined on the computing array, which avoids the data movement between the the feature extraction stage and aggregate stage.
%the data dataflows to handle matrix multiplication in the neural network. These dataflows are categorized into \textit{Weight Stationary}, \textit{Output Stationary} and \textit{No Local Reuse}. 

%More importantly, this data layout should also take into account the iterative graph aggregate dataflow, the key operation of the aggregated stage, to guarantee the seamless combination of the feature extraction and aggregated stage. Thereby, based on these design philosophies and output stationary dataflow, 


\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_map_methods.eps}
\caption{Map strategies.}
\label{fig:Map_strategies}
\vspace{-6pt}
\end{figure}

\begin{table}[]
\centering
\footnotesize
\caption{The analysis of map strategies. The input graph has N vertices with F input feature dimensions. The output feature dimensions is H, and the row and column number of 2D PE array is R and C respectively.}
\label{table:ma}
\begin{tabular}{llll}
\hline
                           &  Latency & Bandwidth & utilization   \\ \hline
 VS   & $N\times F \times H/(R \times C)$ & $R \times C + 1$ &  100\% \\
 VFS  & $N\times F \times H/(R \times C)$ & $R \times C + 1$ &  100\% \\
 HS   & $N\times F \times H/(R \times C)$ & $R + C$ & $[(1-(H\%C)/C, 100\%]$ \\ \hline
\end{tabular}
\end{table}

\subsubsection{The graph property aware dataflow}
As shown in~\autoref{fig:Map_strategies}, since the EnGN adopts 2D PE array, the map methods of the output stationary dataflow has three different strategies: (1) vertex stationary, each output vertex is mapped on the designated PE of the PE-array; (2) vertex's feature stationary, the output feature of one vertex are mapped on the PE-array sequentially; and (3) hybrid stationary, partial feature of some vertices are mapped on the PE-array in designated order. We analyzed the above three strategies from bandwidth, utilization, and latency using the GCN model, which is shown in~\autoref{table:ma}. Note that the PE utilization of the third method is involved with the output feature dimensions $H$, however, in real-world graph application, the dimension of output feature must be maintained within a certain length to avoid information loss. Thereby, we assume that the $H$ is much larger than the number of PE column. Based on this assumption, the compute latency and PE utilization of the three strategies are basically similar while the internal memory bandwidth requirement of the third method is smallest compared to the other two methods. Consequently, based on the hybrid stationary methods, we propose the graph property aware (GPA) dataflow to decouple the input property of the vertex and the hardware computing structure. In this manner, as shown in~\autoref{fig:Architecture details}, each PE in the same column of PE-array is responsible for a single dimension of vertex property and each PE in the same row handles a single vertex. The properties of a vertex are arranged in columns and aligned in the property bank. The dimensions of input vertex property become independent to the hardware architecture and can be continuously injected to the PE-array regardless of the array size and the property dimension. However, as shown in~\autoref{fig:Architecture details}, each column is responsible for generating one dimension of output property while the dimension of output property is determined by the GNN models. Thereby, when the column size of the weight matrix is larger than that of the PE-array, we choose to split the weight matrix into partitions that match the column size of PE-array. For example,~\autoref{fig:Architecture details} depicts the weight matrix with 6 columns and 5 rows while the column size of PE-array is 3, where the row size of weight matrix depends on 5-d property of input vertex and the column size of weight matrix is determined by the target GNN model. In this case, the weight matrix is split by column into two parts to match the column size of PE-array. After that, the two pieces of weight sub-matrix are placed in the weight banks in the order of rows. In this manner, the processing unit can handle vertex with arbitrary dimension property.

%The feature extraction stage maps the high dimensions property of vertices to the low dimensions by using the learned weight matrix, and this stage is simply matrix multiplication operation. Thus, EnGN modifies the classical systolic array architecture to perform the feature extraction stage in NGPU. As shown in~\autoref{fig:Architecture details}, in order to handle arbitrary-dimension property of GNN algorithms, we propose the graph property aware (GPA) dataflow to decouple the input property of the vertex and the hardware computing structure. In this manner, each PE in the same column of PE-array is responsible for a single dimension of vertex property and each PE in the same row handles a single vertex. The properties of a vertex are arranged in columns and aligned in the property bank. The dimensions of input vertex property become independent to the hardware architecture and can be continuously injected to the PE-array regardless of the array size and the property dimension. However, as shown in~\autoref{fig:Architecture details}, each column is responsible for generating one dimension of output property while the dimension of output property is determined by the GNN models. Thereby, when the column size of the weight matrix is larger than that of the PE-array, we choose to split the weight matrix into partitions that match the column size of PE-array. For example,~\autoref{fig:Architecture details} depicts the weight matrix with 6 columns and 5 rows while the column size of PE-array is 3, where the row size of weight matrix depends on 5-d property of input vertex and the column size of weight matrix is determined by the target GNN model. In this case, the weight matrix is split by column into two parts to match the column size of PE-array. After that, the two pieces of weight sub-matrix are placed in the weight banks in the order of rows. In this manner, the processing unit can handle vertex with arbitrary dimension property.
\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_EnGN_hardware_details.eps}
\caption{Architecture details.}
\label{fig:Architecture details}
\vspace{-6pt}
\end{figure}
\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_edge_balance.eps}
\caption{Edge rearrange.}
\label{fig:edge_rearrange}
\vspace{-6pt}
\end{figure}
\subsubsection{The Ring Edge Reduce topology for PE communication} 
The aggregate procedure needs to collect the information according to the edge information. Thereby, as shown in~\autoref{fig:Architecture details}, each row of the PE-array in NGPU possesses a dedicated edge bank and each PE in the same row receives the same control signal parsed from edge list in the graph to gather the corresponding vertex property. Meanwhile, because each PE needs to broadcast its own vertex features generated by the feature extraction stage to all other PEs in the same column, aggregating the received information simultaneously can result in a large amount of hardware resource and power consumption. Thereby, inspired by the ring-all-reduce concept~\cite{ringreduce}, we propose the ring-edge-reduce (RER) aggregate dataflow to conduct aggregate stage inside the PE array instead of moving the data out to the buffer. As shown in~\autoref{fig:Architecture details}, because each column of PE performs the same operations without any communication in between, each PE in the same column of array is connected to its neighbors through an on-chip network of ring topology. Each PE in the same column only communicates with its two nearest neighbors (north, south). In our design, the PE sends its information to the northern neighbors and receives the information sent from the southern neighbors for property aggregating. In this manner, a PE can select the relevant vertices to aggregate based on the control signal parsed from the edges during the information flow across the ring. 

The RER dataflow makes the hardware design simple yet efficient when the graph is dense and the vertex properties flow through the ring are mostly used for aggregation. However, many of the large graphs in practice are sparse and aggregation is inactive in many cases. The RER dataflow example on a sparse graph is shown in~\autoref{fig:edge_rearrange}. The adjacency matrix of the sparse graph is presented on the left side of the figure. The computing array is assumed to be $3 \times 3$. In cycle 0, three edges from different edge banks will be fetched and the properties of $V_0$, $V_1$ and $V_2$ will flow across the ring at the same time. It takes the RER three cycles to complete the aggregation on $V_0$, $V_1$ and $V_2$. Similarly, it also takes RER another three cycles to aggregate on $V_3$, $V_4$ and $V_5$. In this manner, many of the aggregation is inactive due to the graph sparsity. the flow of the first three vertex properties. of the RER, PE can only deal with three edges (green) on the diagonal of the adjacency matrix, followed by the edges with blue and orange color. However, ~\autoref{fig:edge_rearrange} depicts only the first PE is active while the other two in idle. The reason PE underutilization is that the sparse of the graph makes the edge process tasks on each PE unbalanced. More importantly, the power-law distribution of real-world graphs also aggravates the operation imbalance problem. To address this issue, as shown in~\autoref{fig:Map_strategies}, we propose edge recombination technology to alleviate the workload imbalance problem at aggregate stage. Edge recombination shuffles the edge list of the graph first, and then extracts edges from the shuffled edge list to construct a new edge list according to the direction of RER dataflow and the source and destination vertex id of the edge. Meanwhile, the shrink of vertex output feature dimensions enables accelerator to store more vertices with output feature compared to vertices with input feature in the same storage capacity, which also provides an opportunity for edge recombination. In this manner, accelerator can process edges of the graph with high utilization, as shown in~\autoref{fig:Map_strategies}.

\subsection{The On-chip Memory Hierarchy}
\textbf{PE register file} The register files (RF) equipped in the PEs are divided into four groups including source vertex groups(SRC RF), destination vertex groups (DST RF), and two shadow groups (Shadow RF), which is depicted in~\autoref{fig:Memory hierarchy}. The SRC RF stores the source vertex values generated in the feature extraction stage. The DST RF stores the destination vertex feature updated during the aggregate and update stages. In addition, there are two programmer-invisible Shadow RFs holding the SRC and DST vertex values previously generated by the PEs of the same column, which work together with the DST and SRC RFs in a ping-pong way. 
\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/5_level_cache.eps}
\caption{Memory hierarchy.}
\label{fig:Memory hierarchy}
\vspace{-7pt}
\end{figure}

\textbf{Multiple-level caches} The real world graph has up to millions of vertices. Although the graph tiling technique adopted by EnGN helps fit the sub-graphs into the on-chip buffer, the set of vertices in the sub-graphs will still outsize the register files of the PE array. Meanwhile, the result banks are used to store the temporary aggregate results. PE frequently accesses the long-latency result bank will result in performance degradation. Thus, to improve the throughput of EnGN, as shown in~\autoref{fig:Memory hierarchy}, we insert a degree aware vertex cache (DAVC) between the result banks and the register file of each PE to improve the performance of the EnGN. The register file, DAVC, and the result banks are regarded as the first, second, and last level memories on chip, respectively. DAVC is a direct-mapped cache with the write-back policy and cache hit time of one cycles. DAVC uses the destination vertex id of edges as the line tag to determine whether the access to the vertex data hit or not in the DAVC. If hit, the vertex data will be directly read to DST RF in the PE unit. Otherwise, EnGN will access the last-level result banks. DAVC adopts the least recently used (LRU) replacement policy~\cite{LRU}. In this manner, the DAVC can alleviate the overhead incurred by the result bank accesses. EnGN also allocates a small space in the DAVC to cache some of the vertices with high-degree to reduce the on-chip memory traffics and the memory bandwidth required by the vertex data refetch because of the power-law distribution in the real-world graph. Since EnGN adopts graph tiling methods with a deterministic strategy, the vertex access can be predicted in advance. Thereby, EnGN provides a prefetcher unit to prefetch the vertices from off-chip memory to replace the property of vertex resides in the result banks as long as the all edges associated with the hold vertex are processed.

%For example, as shown in~\autoref{fig:Memory hierarchy}, suppose the compute array is sized at $1\times3$, EnGN needs to process the $(1,12)$, $(2,18)$, $(0,21)$, and $(1,24)$ edges. Because the number of the destination vertex of these edges can be divided by three, these edges are assigned to the first row $PE(0,0)$. The first edge $(1,12)$ can be directly processed in $PE(0,0)$ because the vertex 12 ($V_{12}$) is hit in the register file. The second edge $(2,18)$ in $PE(0,0)$ entails the access to the result bank because the vertex 18 ($V_{18}$) is not hit in the register file of $PE(0,0)$ and DAVC. In this case, DAVC will read a data chunk that contains multiple vertices from the result bank for better spatial locality. After that, when edge $(0,21)$ is accessed, PE can directly fetch data from DAVC without accessing the result bank with two cycle latency. 

%Considering the real-world graphs are highly skewed and generally follow the power-law distribution and the paper~\cite{AliGraph} also has proven that caching a small number of vertices with high-degree can achieve a significant cost decrease of graph traversals. Thereby, EnGN allocates a small space in the DAVC to cache some of the vertices with high-degree to reduce the off-chip memory traffics and the memory bandwidth required by the vertex data refetch. Meanwhile, Since EnGN splits the large-graph into 2-D partitions with a deterministic strategy, the vertex access can be predicted in advance. Thereby, EnGN provides a prefetcher unit to prefetch the vertices from off-chip memory to replace the property of vertex resides in the result banks as long as the all edges associated with the hold vertex are processed.
%These vertices with high-degree are prefetched from the off-chip memory to DAVC before a graph iteration begins. Until the end of a graph iteration, the data of these vertices with high-degree are written back to off-chip memory.

\textbf{Edge Bank} EnGN adopts graph tiling technique to divide the large graph into intervals and shards~\autoref{sec:graphtiling}. The edges of each shards are divided into different bank using modulo function according to the destination vertex id and the PE array size (\textbf{Edge Hash}), which is shown in~\autoref{fig:Architecture details}. For example, edges $(v_{5}, v_{0})$, $(v_{5}, v_{1})$, $(v_{5}, v_{2})$ will be placed into Row-1, Row-2, and Row-3 of the PE array, respectively. In this manner, each bank is only responsible for some dedicated edges and vertices update operations, heavy write conflicts due to simultaneous updates to the same vertex in different PEs can also be avoided. Meanwhile, we also rearrange the order of the edges within a shards based on the flow direction of the data in the ring topology to avoid redundant data traffics in the ring and improve the processing throughput of the edges.
%since EnGN adopts a ring-edge-reduce strategy to perform the aggregate stage, the processing order of edges within a shard must be orchestrated to avoid redundant data traffics in the ring and improve the processing throughput of the edges. For this reason, we rearrange the order of the edges within a shard according to the flow direction of the data in the ring topology. Edges are firstly sorted by the destination vertex and then sorted by the source vertex. After that, all edges with the same destination vertex in a PE unit are rearrange based on the order of the source vertex arriving at the PE. In this manner, when data flows in the ring, EnGN can guarantee that all edges can be handled in time.

%\begin{figure*}[!t]
%\centering
%%\setlength{\belowcaptionskip}{-10pt}
%\includegraphics[width=2.1\columnwidth]{Image/4_Neural_Graph_processing_model_in_EnGN.eps}
%\caption{Neural graph processing model in EnGN.}
%\label{fig:Neural graph processing model in EnGN}
%\end{figure*}	

\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/4_Dataflow_on_EnGn.eps}
\caption{EnGN Dataflow.}
\label{fig:EnGN Dataflow}
\vspace{-5pt}
\end{figure}

\subsection{EnGN dataflow}
We present in~\autoref{fig:EnGN Dataflow} an example to illustrate the execution flow of a GNN layer on the proposed EnGN hardware architecture based on GCN model~\cite{GCN}. Similar to the EnGN processing model, the execution stage of one GNN layer on the accelerator is also divided into three stages: feature extraction, aggregate, and update stage. The feature extraction and aggregate stage are executed in a pipelined manner while the update stage can only be triggered when the aggregate stage is completed. Without losing generality, as shown in~\autoref{fig:Architecture details} we consider a small design that consists of $4\times3$ PEs and the input graph is the same as the~\autoref{fig:EnGN processing model}. For brevity, we only describe the flow at the $PE(0,0)$ and $PE(1,0)$.

\textbf{Feature extraction:} At Cycle 0, $PE(0,0)$ receives the first dimension of the input vertex $V_0$ property $I(0,0)$ at the layer $l-1$, and the weight data $W(0,0)$ to generate the temporary property result $P(0,0)$. The result are stored in the local register file. 

At cycle 1, $PE(0,0)$ receives the second dimensions of input vertex $V_0$ property $I(0,1)$ and the weight data $W(1,0)$. Both of them are used to update the temporary property result $P(0,0)$.

On the follow-up cycles, the operations on $PE(0,0)$ are similar to cycle 1. The following new input properties $I(0,2)$, $I(0,3)$, $I(0,4)$ and the associated weight data $W(2,0)$, $W(3,0)$, $W(4,0)$ continuously feed into $PE(0,0)$ until the dimensions of vertices have been covered.

At cycle 4, the result $P(0,0)$ is generated and stored into the register file, waiting to be used by the aggregate stage. 

\textbf{Aggregate:} At cycle 5, Since the edge buffer contains vertex 0, $PE(0,0)$ uses $P(0,0)$ to generate the aggregate result $A(0,0)$. At the same time, $PE(0,0)$ sends $P(0,0)$ to $PE(3,0)$ and prepares for receiving the $P(1,0)$ sent from $PE(1,0)$.

At cycle 6, although $PE(0,0)$ receives $P(1,0)$ from $PE(1,0)$, $P(1,0)$ will not be utilized to update $A(0,0)$ because vertex 1 does not exist in the according edge list provided by the edge buffer, which means vertex 1 is not connected to vertex 0. Meanwhile, $PE(0,0)$ send $P(1,0)$ to $PE(3,0)$ and prepares for receiving $P(2,0)$ sent from $PE(1,0)$.

At cycle 7, $PE(0,0)$ receives $P(2,0)$ from $PE(1,0)$ and leverages it to update the aggregate result $A(0,0)$ because vertex 2 is in the according edge list provided by the edge buffer. Meanwhile, $P(2,0)$ is sent to $PE(3,0)$.

At cycle 8, $PE(0,0)$ receives $P(3,0)$ from $PE(1,0)$ and leverages it to update the aggregate result $A(0,0)$. In this case, all vertices have been traversed by each PE. Thus, $A(0,0)$ summarizes all the relevant edge information and will be stored in the register file to wait for the update stage.

\textbf{Update:} At cycle 9, since all edges associated with vertex 0 has been traversed, the aggregate result $A(0,0)$  will not be changed. Thereby, the update stage is triggered, and the aggregate result $A(0,0)$ is processed by the user-defined apply function, i.e. activation function $ReLu(\cdot)$ in GCNs, to generate the result $O(0,0)$ as the input to the next layer $l$. 

==> Section/Engn_framework_abstraction.tex <==
\section{EnGN Overview}
%In this section, we will summarize the common computing patterns of the GNN models and %propose a unified EnGN processing model that can cover general GNNs. Then, we 
%will map the typical GNN models to the proposed EnGN processing model and 
%demonstrate the use of the EnGN model for GNNs.
\setcounter{algorithm}{0}
\begin{algorithm}[t]
%\scriptsize
\footnotesize
   \begin{algorithmic}[1]
	\caption{{EnGN processing model}}
	\label{alg:EnGN-model}
	\Require Graph $G = (V,E)$, Vertex property $Prop$ and $Tmp_{prop}$, layer $l$, learned parameter $W_{feature}, W_{update}$
    \Ensure Vertex Property $Result$
    \For{$l \leftarrow 1 $  to  $l_{max}$}
		\For{each edge $e \in Edge$}
			\State $tmp \leftarrow \textcolor{red!70!black}{\texttt{Feature\ extraction}}(Prop[e.src], Prop[e.dst], W_{feature})$ 
			\State $Tmp_{prop}[e.dst] \leftarrow \textcolor{red!70!black}{\texttt{Aggregate}}(Tmp_{prop}[e.dst],tmp)$
		\EndFor
		\For{each edge $e \in Edge$} 
			\State $Prop[e.dst] \leftarrow \textcolor{red!70!black}{\texttt{Update}}(Prop[e.dst], Tmp_{prop}[e.dst], W_{update})$
		\EndFor
	\EndFor
	    \State $Result \leftarrow Prop$
   \end{algorithmic}
\end{algorithm}
\subsection{EnGN processing model}
As discussed in prior section, GNN models share three common computing patterns. 
Based on the aim of each computing pattern, they can be abstracted as \textit{feature 
extraction}, \textit{aggregate}, and \textit{update}. The \textit{feature extraction} stage condenses the property 
of each vertex in the graph using a neural network. Similar to conventional convolution operations, 
it can refine the high-dimension vertex properties to low-dimension ones for more efficient 
feature representation. The \textit{aggregate} stage embeds the graph topology by accumulating each vertex's  neighbor properties generated in the feature extraction stage to its vertex property with various 
arithmetic operations such as max, min, and add to produce unified output features. The \textit{update} stage leverages learned parameters to further condense the output features obtained in the aggregate stage, then applied a non-linear activation function or GRU/LSTM function to each vertex of the graph before output, making GNN capable to learn and perform more complex tasks. Note that when the aggregate stage adopts sum operation, the learned parameters in the update stage can be computed in the feature extraction stage because of the matrix multiplication associative law. It also provides an opportunity for EnGN to dynamically adjust the stages of matrix operations to optimize EnGN performance, which will be introduced in~\autoref{sec:optimization}.

%The main idea of graph neural network is based on the neighborhood aggregation strategy, which iteratively updates the representation of node by aggregating representation of its neighbors. Based on this concept, we can abstract different graph neural network models into a general GNN framework with three stages: feature extraction, aggregate, and update, which is shown in Algorithm-1. In illustration, the EnGN processing model receives an input graph in the coordinate list (COO) representation. Besides, to support sparse column (CSC) and compressed sparse row (CSR) representation, EnGN is able to convert graphs in CSR and CSC representation to COO format. In COO format, each edge on the graph is represented as a 3-tuple (src, dst, value), where the value is defined by the users. As shown in Figure 1, the vertex on the graph is associated with a vertex property, where the dimension of vertex property is determined by the dataset and GNN model. Meanwhile, compared to the traditional graph algorithms, GNN algorithms need the learned weight parameters to refine the property of vertex during the graph iterative processing. In each iteration, the computation can be divided into three stages: Feature extraction, Aggregate, and Update. The feature extraction stage extracts the property of each vertex on the graph using a neural network, which can map the high-dimension property of vertex into low-dimension features to preserves more property information at a lower cost. The aggregate stage accumulates neighbors features of vertex in the graph generated from the feature extraction stage to produce a unified result on vertex according to the edge information in the graph. Meanwhile, the aggregate stage applies various arithmetic operations such as max, min, and add, to these neighbors features to embed the graph topology into the property of vertex. The update operator applies vertex feature generated from the aggregate stage to the non-linear activation function or GRU/LSTM function, enabling GNNs to learn and perform more complex tasks.

On top of the abstraction, we propose a unified EnGN processing model that can cover general GNN models 
using the common computing functions as shown in \autoref{alg:EnGN-model}. Suppose the graph is 
represented as $G(V, E)$ where $V$ and $E$ represent the set of vertices and edges in the graph respectively.The
$Property$ is the set of vertex property of the graph. By default, the input graph is stored as a coordinate list (COO). 
Each edge in the graph is a tuple ($src$, $dst$, $val$), where $val$ usually stands for the edge property and it depends on graph definition. 
The EnGN execution flow follows the neighborhood aggregation strategy, which iteratively updates the 
representation of vertices by aggregating representations of their neighbors. Since all the vertices 
in the graph will be processed in each iteration for GNN algorithms, EnGN is organized and presented as an edge-centric processing model 
to ensure more efficient memory accesses~\cite{Edge_centric}. 

For each edge, both the source vertex property and the destination vertex property are condensed with 
$W_{feature}$ using $feature\_extraction(\cdot)$ to obtain a temporary property $tmp$.
Then the $tmp$ is added to the destination property using $aggregate(\cdot)$ function.
Since there may be multiple edges that are incident to the same destination vertices, $aggregate(\cdot)$ 
is essentially a reduce function. When all the destination vertices are reduced, the 
activation function and sometimes the followed user-defined non-linear operator such as LSTM or GRU layer with learnable weights $W_{update}$ are used to filter the output using $update(\cdot)$ for high-level computing tasks such as node classification, and link prediction. 

%Then for all incoming edges, some GNN algorihtms needs the property of destination vertex $dst.prop$. Then, the corresponding vertex property is processed int the \texttt{Feature extraction} stage with associated weight data $Weight_{vertex}$ and performs aggregate operations in the \texttt{Aggregate} to a form single value.  Lastly, \texttt{Update} stage applies application-specific function to update the property of each vertex and the propety generated in the \texttt{Aggregate} using associated weight data $Weight_{feature}$.    \cheng{Try to explain the algorithm using the pseudo code.}

To help understand the EnGN execution model, we present a vivid example of GCN~\cite{GCN} processed by the EnGN architecture
as shown in~\autoref{fig:EnGN processing model}. Suppose an input graph has four vertices and 
each vertex has a 5-dimension property. The input property of the vertices are denoted 
as $I^{v_0}$, $I^{v_{1}}$, $I^{v_{2}}$, $I^{v_{3}}$.
In $feature\_extraction(\cdot)$ function, the feature extraction function takes both the vertex 
property i.e. $I^{v_0}$, $I^{v_{1}}$, $I^{v_{2}}$, $I^{v_{3}}$ and associated 
weight matrix $W_{vertex}$ as input. Then it has the weight matrix multiplied with 
the high-dimension input vertex property to generate low-dimension temp features. 
Note that the size of the weight matrix is associated with both the input property dimension 
and output temp feature dimension. In this example, the size of the weight matrix is $5\times3$. 
With the feature extraction function, the input vertex properties are converted to 3-dimension 
temp features donated as $P^{v_0}$, $P^{v_{1}}$, $P^{v_{2}}$, $P^{v_{3}}$.
In $aggregate(\cdot)$ function, it receives the results of $feature\_{extraction}$ function 
and aggregates the property of each vertex's incoming neighbors. As shown in~\autoref{fig:EnGN processing model}, 
the temp properties of vertex 2 and 3 i.e. $P^{v_{2}}$, $P^{v_{3}}$ are added to temp property of vertex 0 as vertex 2 and 3 are incoming neighbors of vertex 0 $P^{v_{0}}$ according to the graph topology. When the aggregation processing is done, $update(\cdot)$ starts. It has the vertex features i.e. $P^{v_{0}}$, $P^{v_{1}}$, $P^{v_{2}}$, $P^{v_{3}}$ filtered using an activation function. The filtered output properties donated as $O^{v_{0}}$, $O^{v_{1}}$, $O^{v_{2}}$, 
$O^{v_{3}}$ become the input to the next iteration of GNN processing. 
\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.99\columnwidth]{Image/1_EnGN_processing_model.eps}
\caption{Overview of EnGN processing.}
\label{fig:EnGN processing model}
\end{figure}

Similar to the GCN, we further have the rest of the typical GNN algorithms mentioned in~\autoref{sec:section_2} mapped 
to the EnGN processing model.~\autoref{table:GNN algorithms on GNN framework} summarizes the resulted EnGN processing 
functions.

--------------------------------------------------------------------------------

\section{Motivation}
\subsection{Workload characterization}
To gain insight of the computing characteristics of GNN processing models, we leverage the state-of-the-art GNN software framework, DGL, to analyze the five aforementioned GNN models on Intel Xeon CPU. \autoref{fig:execution time} shows the execution time breakdown of GCN, GS-POOL, R-GCN, Gated-GCN, and GRN on the  datasets that are selected from~\autoref{table:dataset}. The feature extraction, aggregate, and update stage occupy a significant amount of execution time illustrates the need for acceleration. \autoref{fig:execution time} depicts that the feature extraction and update stage that mainly involves vector, tensor, and element-wise operations consumes less time than aggregate stage that mainly involves message-passing over the graph structure on the Cora, PubMed dataset while the Cora-Full dataset appear reverse phenomenon. To explain this phenomenon, firstly, we analysis the behavior of the three stage on the Xeon CPU. \autoref{table:exec_pattern} identifies the feature extraction and update stage is compute-intensive and performs regular computation and memory access because they gain high cache hit ratio and less memory accesses from DRAM. However, the aggregate stage is message-intensive and suffers from dynamic computation and irregular memory access because they suffer from high cache miss ratio and abundant ineffectual memory accesses from DRAM. Therefore, compared to dataset with short property length, such as Cora and PubMed, Cora-Full with long property length results in higher operations in the feature extraction and update stage, which causes higher execution time compared to aggregate stage.

\begin{figure}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=0.9\columnwidth]{Image/Time_breakdown.eps}
\caption{Execution time breakdown of GNN model.}
\label{fig:execution time}
\vspace{-10pt}
\end{figure}


\begin{figure*}[!t]
\centering
%\setlength{\belowcaptionskip}{-10pt}
\includegraphics[width=1.99\columnwidth]{Image/TC_factors.eps}
\caption{The factors that impacts the performance of the GCN on synthetic data. (a) Varied input feature length of the vertex. (b) Varied output feature length of the first GCN layer. (c) Varied edge to vertex ratio of the graph.}
\label{fig:factors}
\vspace{-10pt}
\end{figure*}

\begin{table}[!t]
    \scriptsize
    %\footnotesize
    %\small
    \centering
    \setlength\tabcolsep{4pt}
    \setlength{\belowcaptionskip}{0pt}
    \setlength{\abovecaptionskip}{0pt}
    \caption{Execution pattern of GCN on Dataset}
    \label{table:exec_pattern}
\begin{tabular}{ccccc}
\hline
\textbf{}                                                                             & \textbf{Feature extraction} & \textbf{Aggregate} & \textbf{Update}             \\ \hline
\textbf{IPC}                                                                          & 1.73                        & \textbf{0.77}      & 0.97                        \\
\textbf{L3 cache miss ratio}                                                          & 56.60\%                     & \textbf{82.62\%}   & \multicolumn{1}{c}{46.47\%} \\
\textbf{\begin{tabular}[c]{@{}c@{}}CPU stalls caused by \\ memory loads\end{tabular}} & 15.16\%                     & \textbf{40.8\%}    & 30.15\%                     \\
\textbf{DRAM energy}                                                                  & \textbf{0.018}              & \textbf{0.008}     & 0.001                       \\ \hline
\end{tabular}
\end{table}

\begin{table}[!t]
    \scriptsize
    \centering
    %\footnotesize
    %\small
    \setlength\tabcolsep{4pt}
    \setlength{\belowcaptionskip}{0pt}
    \setlength{\abovecaptionskip}{0pt}
    \caption{Exchangeability of execution flow on GCN}
    \label{table:flow}
\begin{tabular}{cccc}
\hline
\textbf{}                    & \textbf{Feat to Agg} & \textbf{Agg to Feat} & \textbf{Reduction} \\ \hline
\textbf{Data access (bytes)} & 226368               & 15575312             & 68.81x             \\
\textbf{Operations}           & 168896               & 15126748             & 89.56x             \\
\textbf{Execution time on CPU (ms)} & 2705.114             & 113190.5037          & \textbf{41.84x}    \\ \hline
\end{tabular}
\end{table}

Based on this observation, we further exploit the mainly factor that affect the execution time of the three stages on the same graph: 1) input property length, 2) output property length, and 3) edge-to-vertex ratio. \autoref{fig:factors} illustrates the first two mainly affects the feature extraction and update stage because they determine the size of the weight, which represents the total number of operations. Meanwhile, \autoref{fig:factors} also depicts the middle and the last affects the aggregate stage. The reason is that, the output property will be used in aggregate stage, which determines the total number of accumulate or element-wise operations in aggregate stage. In addition, the edge-to-vertex ratio represents the sparsity of the graph, which impacts the volume of message information in aggregate stage. Since the output property length impacts the performance of the aggregate stage, We further analyze the impact of the execution flow of the three stages on performance. \autoref{table:flow} shows that, when input property length is larger than output property and operator in aggregate is the sum, the execute feature extraction stage ahead of the aggregate stage can reduce data access and computation of aggregate stage without affecting the final result. In contrast, the aggregates stage ahead of the feature extraction stage is a better choice. 

In summary, the feature extraction and update stage are compute-bound while the aggregate stage is memory-bound, which guides us to improve parallelism to accelerate feature extraction and update stage and reduce unnecessary memory accesses to accelerate the aggregate stage. Meanwhile, the three factors that impact the performance of three stages and the interchangeability of the execution sequence also provides optimization space for accelerator design.

\subsection{GNNs inefficiencies on hardware architecture}
\textbf{Inefﬁciencies of CPUs\&GPUs} The cache hierarchy and data prefetching technology of current CPUs struggle in fully utilizing data reuse of the aggregate stage due to its irregularity compute pattern and random memory access. Similarly, GPUs optimized for compute-intensive workloads with regular execution pattern encounters workload imbalance, memory divergence and branch divergence in the aggregate stage due to its irregularity. Meanwhile, GPUs also suffer from costly data copy and thread synchronization. 

\textbf{Inefﬁciencies of DNN\&Graph accelerator} The deep learning accelerators (DLA) are designed to carry out the inference dataflow of deep neural network on regular data structure such as image or audio, but they do not naturally and efficiently express the graph structure and the graph propagation dataflow. Even though some GNN models can be represented as an adjacent matrix multiplication operation, it still cannot be efficiently executed on sparse deep learning accelerators. This is because the source of sparsity of GNN comes from input graph while DNN from weight, the degree of sparsity of GNN is larger than 99\%, which is higher than the sparsity of weight (50\%) adopted by DNN, and the distribution of sparsity of GNN follows power-law while the distribution of DNN is roughly balanced. As for graph accelerators~\cite{NUMA-aware},~\cite{GraphMat}, they can support the graph propagation model but it is unable to carry out the computation pattern for the neural network inference, such as tensor multiplication, convolution, and activation function. Although Graphiciondao~\cite{Graphicionado} and GraphGen~\cite{GraphGen} are designed to provide general application-specific graph acceleration with hardware. For example, Graphiciondao provides a vertex program specification with user-defined operators. However, it takes non-trivial efforts to provide appropriate computational abstraction for GNN algorithms under the Graphicicondao framework. More importantly, Graphicicondao falls short in handling the high-degree vertex/edge data incurred by the power-law distribution of graph, which results in redundant memory accesses and high energy consumption. Meanwhile, compared to traditional graph algorithms with small and invariant property, graphs on GNN algorithms have a high-dimension and dynamic vertex property, which is not considered on traditional graph accelerators.

\textbf{Inefficiencies of State-of-the-art} Due to the inefficiency of DNN and graph accelerator, a tailored GCN accelerator, HyGCN, is presented. HyGCN abstracted the execution process of the GCN model to aggregation and combination stage and tailored corresponding aggregation and combination hardware engine to perform GCN acceleration, where the aggregation and combination engine is designed to solve the irregularity operation and the regular operation of GCN, respectively. Despite HyGCN solved the hybrid computational pattern of GCN, it still suffers from non-universal and computational inefficiency. The reason is attributed to four factors. First, the programming model of HyGCN is designed for GCN, a type of GNN models, limiting their applicability to various GNN models. Second, the aggregation and combination engine of HyGCN adopts the separation design, which brings extra write and read operation of on-chip memory. Meanwhile, HyGCN leveraged SIMD cores to perform aggregation on each vertex by using this vertex's neighbors. It overlooks the inherent reusability of intermediate data, bringing extra energy consumption incurred by the compute unit up to x\%. Third, HyGCN only focuses on the relatively small datasets with only less than million vertices and billion edges while the real-world graph usually has a million vertices and billion edges. Meanwhile, HyGCN ignores the potential data reusability brought by the power-law distribution of the big real-world graph. Finally, HyGCN ignores the variability of external memory accesses brought by the grid partition methods adopted by HyGCN because the order of the grid execution essentially affects the data reuse and the number of external memory accesses accordingly.


the power-law distribution of the big real-world graph challenges the existing memory hierarchy and caching policy of CPUs and GPUs, for the sparsely distributed high-degree vertices on the graphs makes it hard to reuse the graph data for the conventional architectures.


HyGCN also ignores the data reusability power-law distribution of real-world graph, 





To overcome the above inefficiencies, first, we integrate the computation abstractions required by neural networks and the graph iteration model required by graph processing into the a unified architecture. The computation abstraction provides enough compute capability and flexibility for neural networks, and also provides the graph iteration model that furnishes the capability of high-throughput graph iterative processing in the scatter-and-gather way. In addition, under the scheduling of ring-edge-reduce and graph property aware dataflow, EnGN achieves high GNN processing throughput. Second, EnGN contains a dedicated on-chip memory hierarchy to exploit the vertex locality of data processing in sparse graphs, which can effectively reduce off-chip memory access and the resulted energy consumption. 

 


==> Section/algorithms.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\setcounter{algorithm}{0}
\begin{algorithm}[t]
\scriptsize
   \begin{algorithmic}[1]
	\caption{{EnGN processing model}}
	\label{alg:EnGN-model}
	%\State \textbf{Property}  $Src_{prop}$, $Dst_{prop}$, $Temp_{prop}$
	%\State \textbf{Weight}    $Weight$
	%\State \textbf{Edge}      $Edge$
	%\State \textbf{Result}    $Result$
	\For{each vertex $v \in V$} 
		\State $src.prop        \leftarrow Src_{prop}[v]$
		\State $\textbf{Edge} \ edge\_     \leftarrow Edge[v]$
		\For{each edge $e \in edge\_$}
			\State $dst.prop  \leftarrow Dst_{prop}[e.dst]$
			\State $temp.prop \leftarrow \textcolor{red}{Feature \ Extraction}(src.prop, dst.prop, Weight_{vertex})$
			\State $Temp_{prop}[e.dst] \leftarrow  \textcolor{red}{Aggregate}(Temp_{prop}[e.dst], temp.prop)$
		\EndFor
	\EndFor
	\For{each vertex $v \in V$}
		\State $src.prop  \leftarrow Src_{prop}[v]$
		\State $Result[v] \leftarrow \textcolor{red}{Update}(src.prop, Temp_{prop}[v], Weight_{feature})$
	\EndFor
   \end{algorithmic}
\end{algorithm}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\setcounter{algorithm}{0}
\begin{algorithm}[t]
\scriptsize
   \begin{algorithmic}[1]
	\caption{{EnGN processing model}}
	\label{alg:EnGN-model}
		\For{each edge $e \in Edge$}
			\State $temp.prop \leftarrow \textcolor{red}{Feature\ extraction}(prop_{e.src}, prop_{e.dst}[Optional], Weight_{vertex})$ 
			\State $Temp_{prop}[e.dst] \leftarrow \textcolor{red}{Aggregate}(Temp_{prop}[e.dst],temp.prop)$
		\EndFor
		\For{each edge $e \in Edge$} 
			\State $Result[e.dst] \leftarrow \textcolor{red}{Update}(prop_{e.dst}, Temp_{prop}[e.dst], Weight_{feature})$
		\EndFor
   \end{algorithmic}
\end{algorithm}

\begin{table}[]
\begin{tabular}{|ccccc}
\hline
Dataset   & Vertex  & Edge      & \begin{tabular}[c]{@{}c@{}}Featrue\&\\ Relation\end{tabular} & Label \\ \hline
Cora      & 10858   & 10858     & 1433                                                         & 7     \\
PubMed    & 19717   & 88651     & 500                                                          & 3     \\
Cora-Full & 19793   & 65311     & 8710                                                         & 67    \\
Reddit    & 232965  & 114615892 & 602                                                          & 41    \\ \hline
AIFB      & 8285    & 29043     & 91                                                           & 4     \\
MUTAG     & 23644   & 192098    & 47                                                           & 2     \\
BGS       & 333845  & 2166243   & 207                                                          & 2     \\
AM        & 1666764 & 13643406  & 267                                                          & 11    \\ \hline
\end{tabular}
\end{table}


Meanwhile, considering the real-world graphs are highly skewed and generally follow the power-law distribution, the vertex with high-degree of connectivity will be frequently accessed. Meanwhile, the paper~\cite{AliGraph} has proven that caching a small number of vertices with high-degree can achieve a significant cost decrease of graph traversals. Thereby, in order to reduce the off-chip memory traffics and the memory bandwidth required by the vertex data refetch, EnGN also allocates a small space in the DAVC to cache some of the vertices with high-degree. The reason for allocate space in result banks is the limited size of PE array cannot support large output dimensions of vertex property, thereby, these property values are cached in result banks. When the PE unit accesses these properties, it will replace all property data in the DAVC. These vertices are prefetched from the off-chip memory to DAVC and result banks before a graph iteration begins and some of them are prefetched to the DAVC in a graph iteration. Meanwhile, when EnGN fetches data from off-chip memory and PE unit fetches data from the result banks during a graph iteration, these vertices will be ignored. Until the end of a graph iteration, the data will be written back to off-chip memory.看不懂这一段



\setcounter{algorithm}{0}
\begin{algorithm}[t]
\scriptsize
   \begin{algorithmic}[1]
	\caption{{Edge Rearrange in a Shard}}
	\label{alg:Edge rearrange}
		\State $Edge \leftarrow$ Sort Edge by $e.dst$ 
		\State $Edge \leftarrow$ Sort Edge by $e.src$
		\For{each edge $e \in$ Edge}
		    \For{all edges with the same $e.dst$}
		        \If{$e.src \bmod PE.row < e.dst \bmod PE.row$}
		            \State $E.low \leftarrow e$
		        \Else
		            \State $E.high \leftarrow e$
		        \EndIf
		        \State $Edge \leftarrow {E.high, E.low}$
		    \EndFor
		\EndFor
   \end{algorithmic}
\end{algorithm}

Meanwhile, considering LRU policy attains the frequency of the vertex while it cannot discriminate well between frequently and infrequently. More importantly, the power-law distribution of real-world graphs makes the vertex with high-degree will be frequently accessed, which means frequency is a important attribute in GNN algorithms. Thereby, 

Meanwhile, due to vertices with high-degree cached in the DAVC are not be fetched from off-chip memory during graph iteration, DAVC can also save off-chip memory energy consumption about 15.29\% and 25.74\% compared to the scheme without caching vertices with high degree

Besides, it is known that the substantial computational overhead of neural networks challenges the throughput of CPUs while the irregular graph data structures make it hard to perform parallel GNN computation efficiently on GPUs~\cite{NeuGraph:Parallel}.

 For example, assume the PE array is $5\times 1$ and $PE(2,0)$ need to process edges $(0,2)$,$(1,2)$,$(3,2)$,$(4,2)$. The data flows from south to north in the RER PE array, when the data of $PE(3,0)$ arriving, edge $(0,2)$ occupies the head of the edge queue, resulting in edge $(3,2)$ can not be handled in time. Thereby, we rearrange the edge list to $(3,2)$, $(4,2)$, $(0,2)$, $(1,2)$ according the flow direction of the data in RER PE array.
 
 Meanwhile, when EnGN fetches vertex property data from off-chip memory to the EnGN during a graph iteration, these vertices will be ignored.
 
 In addition, the edge data is also strategically compressed~\cite{GraphH} to balance the edge-induced workloads on each PE and optimized based on hashed edge data layout in the PE array to avoid memory conflicts.
 
 Meanwhile, for RGCN models, the proposed DAST strategy can reduce the operation by 1.58x on average compared to other two fixed strategy FAU and AFU on all knowledge datasets. The reason why the performance boost is lower is that the graph is more sparsity and the dimension of vertex property is low.
 
 LRU policy attains the recency of the vertex while it cannot discriminate well between frequently and infrequently. The power-law distribution of real-world graphs makes the vertex with high-degree will be frequently accessed, which means frequency is a important attribute in GNN algorithms. LFU policy considers the frequency of vertex while it cannot distinguish between vertex that occurred far back in the past and the more recent ones in recording the frequency. Whereas, 
 
 : 1) the vertices selected using FIFO strategy are rarely to be accessed, and 2) 
